Relevance of Ge incorporation to control the physical behaviour of point defects in kesterite

To reduce the prominent VOC-deficit that limits kesterite-based solar cells efficiencies, Ge has been proposed over the recent years with encouraging results, as the reduction of the non-radiative recombination rate is considered as a way to improve the well-known Sn-kesterite world record efficiency. To gain further insight into this mechanism, we investigate the physical behaviour of intrinsic point defects both upon Ge doping and alloying of Cu2ZnSnS4 kesterite. Using a first-principles approach, we confirm the p-type conductivity of both Cu2ZnSnS4 and Cu2ZnGeS4, attributed to the low formation energies of the VCu and CuZn acceptor defects within the whole stable phase diagram range. Via doping of the Sn-kesterite matrix, we report the lowest formation energy for the substitutional defect GeSn. We also confirm the detrimental role of the substitutional defects XZn (X=Sn,Ge) acting as recombination centres within the Sn-based, the Ge-doped and the Ge-based kesterite. Finally, we highlight the reduction of the lattice distortion upon Ge incorporation resulting in a reduction of the carrier capture cross section and consequently a decrease of the non-radiative recombination rate within the bulk material.

==> packages.tex <==
%\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}   
\usepackage[lofdepth,lotdepth]{subfig}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{titlesec}
\usepackage{color}
\usepackage[font=small,justification=justified]{caption}
\usepackage{xurl}
\usepackage{systeme}
\usepackage{listings}
\usepackage{amsmath} %for math greek letters
\usepackage{bm}        % for math
\usepackage{amssymb}   % for math
\usepackage{graphicx}  % needed for figures
\usepackage{dcolumn}   % needed for some tables
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\usepackage{colortbl}
\usepackage{float} % Required for tables and figures in the multi-column environment - they need to be placed in specific locations with the [H] (e.g. \begin{table}[H])
%\usepackage{tabu} %Control of the tabularx vertical spacing
\usepackage{tabularx} %table latex
\usepackage{array}
\usepackage{multirow}
\usepackage{makecell} % for tabular
\usepackage{lettrine} % The lettrine is the first enlarged letter at the beginning of the text
\usepackage{paralist} % Used for the compactitem environment which makes bullet points with less space between them
\usepackage{titlesec} % Allows customization of titles
\usepackage{footnote}
\usepackage{fancyhdr} % Headers and footers
\usepackage{pdfpages}
\usepackage{comment}
\usepackage{hyperref}
\hypersetup{pdfstartview={XYZ null null 1.00}, % 100% zoom
						pdfpagemode=UseNone,  % bookmarks closed
						colorlinks=true,
						citecolor=blue,
						linkcolor=black
}
\usepackage[all]{hypcap} % correct hyperref to figures
\usepackage{booktabs}
\usepackage{afterpage}
\usepackage{capt-of}% or use the larger `caption` package
\usepackage{lipsum}% dummy text
\usepackage{rotating} %to be able to rotate a table 
\usepackage{physics}
\usepackage{wrapfig}

